DuplexJail: Spoken Interruption Attacks on Full-Duplex Speech Models

Full-duplex speech models accept user speech while generating responses, making input timing a potential safety concern. We introduce DuplexJail, which delivers fixed, request-independent spoken jailbreak prompts through the user audio channel. Across four open-source models and 720 harmful requests from AdvBench and HarmBench, we compare fixed-delay and refusal-triggered interruption with request-end and post-response controls. On AdvBench, Guided Completion at a 1.0 s delay raises whole-response attack success rates to 40.3% for PersonaPlex and 48.7% for PersonaPlex-RL, increases of 33.8 and 39.3 percentage points over baseline. On HarmBench, which was not used for prompt selection, the same prompt at a 0.5 s delay increases ASR by 14.7 and 12.3 points, respectively. Effects vary across models: selected conditions increase FLM-Audio's harmfulness, while BayLing-Duplex shows decreases. These results show that spoken-jailbreak effectiveness depends on delivery timing and motivate safety evaluation across stages of full-duplex interaction.

==> tables/tab_different_timing.tex <==
% \begin{table*}[t]
% \centering
% \caption{Late injection. Harmful \%, and in parentheses the difference in points against the no-interruption baseline.}
% \label{tab:late}
% \setlength{\tabcolsep}{4pt}
% \footnotesize
% \begin{tabular}{lcccccc}
% \toprule
%  & \multicolumn{3}{c}{``Sure. Here's how.} & \multicolumn{3}{c}{``Alright, so walk me through} \\
%  & \multicolumn{3}{c}{Step one is''} & \multicolumn{3}{c}{it, you begin by''} \\
% \cmidrule(lr){2-4}\cmidrule(lr){5-7}
% Model & 2\,s & 4\,s & 10\,s & 2\,s & 4\,s & 10\,s \\
% \midrule
% PersonaPlex
%     & 19.2 ($+10.4$) & 15.2 ($+6.3$)  & --
%     & 47.7 ($+38.8$) & 36.5 ($+27.7$) & 27.3 ($+20.8$) \\
% PersonaPlex-RL
%     & 21.9 ($+9.4$)  & 23.1 ($+10.6$) & --
%     & 47.9 ($+35.4$) & 36.3 ($+23.8$) & 28.4 ($+19.0$) \\
% FLM-Audio
%     & 21.5 ($-2.3$)  & 25.4 ($+1.5$)  & --
%     & 23.3 ($-0.6$)  & 25.0 ($+1.2$)  & 19.7 ($+0.4$) \\
% BayLing
%     & 3.1 ($-26.0$)  & 10.8 ($-18.3$) & --
%     & 9.2 ($-32.1$)  & 20.2 ($-21.0$) & 41.9 ($+0.6$) \\
% \bottomrule
% \end{tabular}
% \end{table*}
